Contract Usage and Evolution in Android Mobile Applications

Formal contracts and assertions are effective methods to enhance software quality by enforcing preconditions, postconditions, and invariants. Previous research has demonstrated the value of contracts in traditional software development contexts. However, the adoption and impact of contracts in the context of mobile application development, particularly of Android applications, remain unexplored. To address this, we present the first large-scale empirical study on the presence and use of contracts in Android applications, written in Java or Kotlin. We consider different types of contract elements divided into five categories: conditional runtime exceptions, APIs, annotations, assertions, and other. We analyzed 2,390 Android applications from the F-Droid repository and processed more than 51,749 KLOC to determine 1) how and to what extent contracts are used, 2) how contract usage evolves, and 3) whether contracts are used safely in the context of program evolution and inheritance. Our findings include: 1) although most applications do not specify contracts, annotation-based approaches are the most popular among practitioners; 2) applications that use contracts continue to use them in later versions, but the number of methods increases at a higher rate than the number of contracts; and 3) there are many potentially unsafe specification changes when applications evolve and in subtyping relationships, which indicates a lack of specification stability. Our findings show that it would be desirable to have libraries that standardize contract specifications in Java and Kotlin, and tools that aid practitioners in writing stronger contracts and in detecting contract violations in the context of program evolution and inheritance.

==> data/rq1/contractsByGroup.tex <==
% TABLE GENERATED BY contractstudy.scripts.AnalyseContractUsage
% TIMESTAMP:   Tue Mar 28 23:30:31 WEST 2023
\begin{table}[]
\centering
\caption{Contract elements by type}
\label{tab:contractsbytype}
\begin{tabular}{| c | c | c | c | c | c | c | c |} \hline
type & category & \multicolumn{2}{ c |}{contracts (all ver.)} & \multicolumn{2}{ c |}{contracts (latest)} & \multicolumn{2}{ c |}{contracts (programs)} \\ 
\cline{3-8}
& & Java & Kotlin & Java & Kotlin & Java & Kotlin \\
\hline
	assert & assertion & 0 & 3 & 0 & 3 & 0 & 1 \\ 
	cond. runtime exc. & runtime exception & 0 & 0 & 0 & 0 & 0 & 0 \\ 
	unsupp. op. exc. & runtime exception & 0 & 0 & 0 & 0 & 0 & 0 \\ 
	guava precond. & api & 0 & 4 & 0 & 2 & 0 & 1 \\ 
	spring assert & api & 0 & 0 & 0 & 0 & 0 & 0 \\ 
	commons validate & api & 0 & 0 & 0 & 0 & 0 & 0 \\ 
	JSR303, JSR349 & annotation & 0 & 0 & 0 & 0 & 0 & 0 \\ 
	JSR305 & annotation & 0 & 0 & 0 & 0 & 0 & 0 \\ 
	android & annotation & 40 & 35 & 18 & 18 & 11 & 11 \\ 
	androidx & annotation & 231 & 53 & 194 & 23 & 7 & 7 \\ 
	kotlin contracts & others & 0 & 0 & 0 & 0 & 0 & 0 \\ 
\hline
\end{tabular}
\end{table}


==> data/rq1/contractsGini.tex <==
\begin{table}[]
\footnotesize
\renewcommand\arraystretch{1.1}
\centering
\caption{Gini coefficient by category.}
\begin{tabular}[t]{ccc}
    \hline
    \hline
    Category & Java & Kotlin \\ 
    \midrule
	assertion & 0.70 & 0.71 \\ 
	API & 0.80 & 0.37 \\ 
	annotation & 0.88 & 0.76 \\ 
	CRE & 0.77 & 0.67 \\ 
	others & - & 1.00 \\ 
    \bottomrule
\end{tabular}
\label{tab:contractsGini}
\end{table}

==> data/rq1/dataset.tex <==
% TABLE GENERATED BY contractstudy.scripts.CollectDatasetStats
% TIMESTAMP:   Tue Mar 28 23:24:10 WEST 2023
\begin{table}[]
\centering
\caption{Dataset metrics }
\label{tab:data-metrics}
\begin{tabular}{|l|l|l|l|} \hline
metric & Java & Kotlin & Both \\ \hline
programs & ? & ? &2,354  \\
program versions & ? & ? &4,132  \\
compilation units & 215,769 & 130,402 & 346,171 \\
unparsable compilation units & 440 & - & - \\
\hline
classes & 312,686 & 257,442 & 570,128 \\
methods (all) & 2,151,253 & 655,213 & 2,806,466 \\
constructors (all) & 207,563 & 92,999 & 300,562 \\
methods (public and protected) & 1,838,284 & 534,433 & 2,372,717 \\
constructors (public and protected) & 186,456 & 91,819 & 278,275 \\
KLOC incl comments & 41,373 & 12,746 & 54,120 \\
\hline
\end{tabular}
\end{table}


==> data/rq3/evolution-hierarchy.tex <==
\begin{table}[]
\footnotesize
\renewcommand\arraystretch{1.1}
\centering
\caption{Contract evolution in the context of inheritance.}
\begin{tabular}[t]{ccc}
    \hline
    \hline
    Evolution & Critical & Count \\ \hline
    \midrule
    unchanged & no & 158  \\
    minor change & no & 1  \\
    pre-conditions weakened & no & 3  \\
    post-conditions strengthened & no & 71  \\ 
    \hline
    pre-conditions strengthened & yes & 232  \\
    post-conditions weakened & yes & 0  \\ 
    \hline
    unclassified & ? & 145  \\ 
    \bottomrule
\end{tabular}
\label{tab:evolution-hierarchy}
\end{table}
